Learning Responsibility Allocations for Safe Human-Robot Interaction with Applications to Autonomous Driving

Drivers have a responsibility to exercise reasonable care to avoid collision with other road users. This assumed responsibility allows interacting agents to maintain safety without explicit coordination. Thus to enable safe autonomous vehicle (AV) interactions, AVs must understand what their responsibilities are to maintain safety and how they affect the safety of nearby agents. In this work we seek to understand how responsibility is shared in multi-agent settings where an autonomous agent is interacting with human counterparts. We introduce Responsibility-Aware Control Barrier Functions (RA-CBFs) and present a method to learn responsibility allocations from data. By combining safety-critical control and learning-based techniques, RA-CBFs allow us to account for scene-dependent responsibility allocations and synthesize safe and efficient driving behaviors without making worst-case assumptions that typically result in overly-conservative behaviors. We test our framework using real-world driving data and demonstrate its efficacy as a tool for both safe control and forensic analysis of unsafe driving.

==> misc.tex <==

For ease of notation let $\gamma(\theta) \triangleq \lmat \cos \theta & \sin \theta \rmat^T $. 
Based on \eqref{eq:safety_nonsmooth}, satisfying the constraint: 
\begin{equation}
    % (\zeta - \rho_i)^\intercal\lmat \cos \theta \\ \sin\theta \rmat v \geq - \alpha (h(\mb{x}))
    (\zeta - \rho_i)^\intercal\gamma(\theta) v \geq - \alpha( h (\mb{x}) ), \quad
    \forall \; i \in I_{\rm a}
    \label{eq:uni_cbf}
\end{equation}
is sufficient to guarantee the safety of the system with respect to three dimensional location of the pixel by Theorem~\ref{thm:nonsmooth} \cite{ames_control_2014}. We note that assuming that the initial condition is safe with respect to all $i \in NumPix$, then the control barrier function constraint is always feasible since $v=0$ is always a valid input for any state in the safe set.

In this case the CBF constraint \eqref{eq:uni_cbf} can be rewritten equivalently as: 
\begin{align}
    % (\zeta - \rho_i)^\intercal\gamma(\theta) v & \geq - \alpha( h (\mb{x}) ) \\ 
    v & \leq - \frac{\alpha(h(\mb{x}))}{(\zeta - \rho_i)^\intercal\gamma(\theta) }
    \triangleq p(\mb{x} , \rho_i), \quad
    \forall \; i \in I_{\rm a}.
    \label{acute}
    % \\
    % v + \frac{\alpha(h(\mb{x}))}{(\zeta - \rho_i)^\intercal\gamma(\theta) } &  \geq 0
    % \label{constraint_noLgh}
\end{align}
Equation \eqref{acute} is a consequence of Assumption \ref{assp:FoV} due to the fact that the projection of any point $(\zeta - \rho_i)$ onto the heading direction is negative since $(\zeta - \rho_i) \in {\rm FoV}$ and the $0 < \delta < \frac{\pi}{2} $ forms a field of view of less than $\pi $ radians centered at the heading angle. Thus \eqref{acute}
% \ref{constraint_noLgh}
is sufficient to guarantee safety with respect to pixel $\rho_i$.
% For ease of notation let $p(\mb{x}, \rho_i) \triangleq - \frac{\alpha(h(\mb{x}))}{(\zeta - \rho_i)^\intercal\gamma(\theta) }  $.
% The nonsmooth composed constraint is then: 
% \begin{equation}
%     v \leq p(\mb{x} , \rho_i) , \quad
%     \forall \; i \in I_{\rm a}.
%     % i \in \mathbb{N} \textrm{ s.t. } h(\mb{x}) = h_i(\mb{x}, \rho_i)
% \end{equation}


